Distributed Nonlinear Model Predictive Control for District Heating Networks

This paper presents a distributed nonlinear model predictive control that uses alternating direction method of mul tipliers for district heating networks. Exploiting a graph-based modeling of the thermal dynamics, our controller optimizes the mass flow absorption of buildings in a distributed cooperative scheme that mediates between the superior performance of the centralized control and the privacy preservation of the decentralized schemes. A benchmark three-building network simulation is used to compare the performance of the proposed solution with a decentralized model predictive control scheme.

==> drawings/pressure_balance.tex <==
\begin{circuitikz}
    % First part of the circuit (A)
    
    \draw[dashed] (0,0) -- (0.5,0);
    \draw[dashed] (0,-4) -- (0.5,-4);
    
    \draw (0.5,0) to[short] (1, 0)
        (0.5,-4) to[short] (1, -4)
        (1,-4) to[short, -*] (1,-4)
        (1, 0) to[short, -*] (1,0)
        (1,-1) to[resistor, l=$R_{U}^H$] (1,-3)
        (1,0) to[short, i=$\dot{m}_U^H$] (1, -1)
        (1,-3) to[short] (1, -4);

    \draw(1,0) to[resistor, l=$R_F^B$, i=$\dot{m}_F^B$] (5,0)
        (5,-4) to[resistor, l_=$R_R^B$, i=$\dot{m}_R^B$] (1,-4) 
        (5,-4) to[short, -*] (5,-4)
        (5, 0) to[short, -*] (5,0)
        (5,-1) to[resistor, l=$R_{U}^A$] (5,-3)
        (5,0) to[short, i=$\dot{m}_U^A$] (5, -1)
        (5,-3) to[short] (5, -4)
        (5,0) to[short] (5.5, 0)
        (5,-4) to[short] (5.5, -4);
        
    \draw[dashed] (5.5,0) -- (6,0);
    \draw[dashed] (5.5,-4) -- (6.0,-4);    

    \draw[<-] (0.75,-1) to[bend right=45] node[midway, left] {$\Delta p^{H}$} (0.75,-3);
    \draw[->] (3,-1) to[bend left=90] node[midway, right] {$\Delta p^{H}$} (3,-3);
    
        
\end{circuitikz}

==> drawings/pressure_resistance.tex <==
\begin{circuitikz}
    % Draw the heat producer block
    \draw
    (-3,1) rectangle (0,-7.5)
    node[midway, rotate=90] {Heat Producer};
    
    \draw
    (0,0) to[resistor, l=$R_F^A$, i=$\dot{m}_F^A$] (3,0) % R1
    (3,-1) to[resistor, l=$R_{S1}^A$] (3,-2.5)
    (3,-2.5) to[resistor, l=$R_{S2}^A$] (3,-4)
    (3,-4) to[resistor, l=$R_{S3}^A$] (3,-5.5)
    (0,-6.5) to[resistor, l_=$R_R^A$] (3,-6.5)     
    (3,-6.5) to[short, -*] (3,-6.5)
    (3, 0) to[short, -*] (3,0)
    (3,0) to[short, i=$\dot{m}_U^A$ ] (3, -1)
    (3,-6.5) to[short, -] (3, -5.5)
    
    (3,0) to[resistor, l=$R_F^B$ , i=$\dot{m}_F^B$] (6,0) % R1
    (6,-1) to[resistor, l=$R_{S1}^B$] (6,-2.5)
    (6,-2.5) to[resistor, l=$R_{S2}^B$] (6,-4)
    (6,-4) to[resistor, l=$R_{S3}^B$] (6,-5.5)
    (3,-6.5) to[resistor, l_=$R_R^B$] (6,-6.5)    
    (6,-6.5) to[short, -*] (6,-6.5)
    (6, 0) to[short, -*] (6,0)
    (6,0) to[short, i=$\dot{m}_U^B$ ] (6, -1)
    (6,-6.5) to[short, -] (6, -5.5)

    (6,0) to[resistor, l=$R_F^C$, i=$\dot{m}_F^C$] (9,0) % R1
    (9,-1) to[resistor, l=$R_{S1}^C$] (9,-2.5)
    (9,-2.5) to[resistor, l=$R_{S2}^C$] (9,-4)
    (9,-4) to[resistor, l=$R_{S3}^C$] (9,-5.5)
    (6,-6.5) to[resistor, l_=$R_R^C$] (9,-6.5)    
    (9,0) to[short, i=$\dot{m}_U^C$ ] (9, -1)
    (9,-6.5) to[short, -] (9, -5.5)

    (9, 0) to[short, -*] (9,0)
    (9,0) to[short, -] (12, 0)
    (12,-1) to[short, , i=$\dot{m}_{B}$] (12,-2)
    (12,0) to[resistor, l=$R_{B}$ ] (12,-6.5)
    (9,-6.5) to[short, -] (12, -6.5)
    (9,-6.5) to[short, -*] (9,-6.5); 
    
\end{circuitikz}
